HAT-P-11: Discovery of a Second Planet and a Clue to Understanding Exoplanet Obliquities

HAT-P-11 is a mid-K dwarf that hosts one of the first Neptune-sized planets found outside the solar system. The orbit of HAT-P-11b is misaligned with the star's spin --- one of the few known cases of a misaligned planet orbiting a star less massive than the Sun. We find an additional planet in the system based on a decade of precision radial velocity (RV) measurements from Keck/HIRES. HAT-P-11c is similar to Jupiter in its mass ($M_P \sin{i} = 1.6\pm0.1$ $M_J$) and orbital period ($P = 9.3^{+1.0}_{-0.5}$ year), but has a much more eccentric orbit ($e=0.60\pm0.03$). In our joint modeling of RV and stellar activity, we found an activity-induced RV signal of $\sim$7 m s$^{-1}$, consistent with other active K dwarfs, but significantly smaller than the 31 m s$^{-1}$ reflex motion due to HAT-P-11c. We investigated the dynamical coupling between HAT-P-11b and c as a possible explanation for HAT-P-11b's misaligned orbit, finding that planet-planet Kozai interactions cannot tilt planet b's orbit due to general relativistic precession; however, nodal precession operating on million year timescales is a viable mechanism to explain HAT-P-11b's high obliquity. This leaves open the question of why HAT-P-11c may have such a tilted orbit. At a distance of 38 pc, the HAT-P-11 system offers rich opportunities for further exoplanet characterization through astrometry and direct imaging.

==> tab_rv.tex <==
% time, mnvel, sig_vel, sval, sig_sval, ha, sig_ha, mask
2454335.891030 & 6.50 & 1.03 & 0.5599 & 0.0056 & 0.04539 & 0.00026 &0 \\
2454335.897680 & 6.75 & 1.09 & 0.5614 & 0.0056 & 0.04537 & 0.00026 &0 \\
2454336.746470 & 8.03 & 0.94 & 0.5748 & 0.0057 & 0.04533 & 0.00025 &0 \\
2454336.859340 & 4.30 & 1.03 & 0.5751 & 0.0058 & 0.04531 & 0.00026 &0 \\
2454336.947330 & 0.27 & 1.00 & 0.5765 & 0.0058 & 0.04543 & 0.00027 &0 \\
2454337.729220 & -12.86 & 1.14 & 0.5886 & 0.0059 & 0.04602 & 0.00028 &0 \\
2454337.918740 & -9.76 & 0.96 & 0.5882 & 0.0059 & 0.04556 & 0.00027 &0 \\
2454338.739920 & -14.88 & 0.92 & 0.5925 & 0.0059 & 0.04519 & 0.00025 &0 \\
2454338.918190 & -12.42 & 1.01 & 0.5865 & 0.0059 & 0.04526 & 0.00025 &0 \\
2454339.890660 & -5.94 & 1.03 & 0.5898 & 0.0059 & 0.04528 & 0.00026 &0 \\
2454343.836570 & -18.77 & 1.10 & 0.5833 & 0.0058 & 0.04519 & 0.00027 &0 \\
2454344.966230 & -15.22 & 1.07 & 0.5728 & 0.0057 & 0.04511 & 0.00028 &0 \\
2454396.752330 & -1.43 & 1.12 & 0.5989 & 0.0060 & 0.04517 & 0.00024 &0 \\
2454397.768210 & -1.93 & 1.13 & 0.5925 & 0.0059 & 0.04509 & 0.00024 &0 \\
2454427.728150 & -2.90 & 1.26 & 0.5647 & 0.0056 & 0.04509 & 0.00024 &0 \\
2454428.696400 & 4.89 & 1.58 & 0.5560 & 0.0056 & 0.04489 & 0.00021 &0 \\
2454430.697860 & -8.48 & 1.33 & 0.5511 & 0.0055 & 0.04495 & 0.00023 &0 \\
2454454.708830 & -14.84 & 1.58 & 0.5416 & 0.0054 & 0.04514 & 0.00022 &0 \\
2454455.699230 & -18.00 & 1.39 & 0.5466 & 0.0055 & 0.04503 & 0.00022 &0 \\
2454456.691170 & -16.85 & 1.51 & 0.5370 & 0.0054 & 0.04500 & 0.00023 &0 \\
2454457.688140 & -6.04 & 1.56 & 0.5376 & 0.0054 & 0.04500 & 0.00022 &0 \\
2454460.728800 & -18.84 & 1.66 & 0.5514 & 0.0055 & 0.04524 & 0.00022 &0 \\
2454549.096270 & -9.89 & 1.27 & 0.5173 & 0.0052 & 0.04458 & 0.00025 &0 \\
2454549.134440 & -7.29 & 1.29 & 0.5204 & 0.0052 & 0.04485 & 0.00024 &0 \\
2454602.011840 & -5.35 & 1.05 & 0.5612 & 0.0056 & 0.04486 & 0.00022 &0 \\
2454602.118060 & -2.24 & 1.22 & 0.5580 & 0.0056 & 0.04517 & 0.00024 &0 \\
2454602.948440 & 1.43 & 1.21 & 0.5653 & 0.0057 & 0.04523 & 0.00024 &0 \\
2454603.007660 & 2.37 & 1.14 & 0.5641 & 0.0056 & 0.04523 & 0.00024 &0 \\
2454603.119350 & 1.13 & 1.20 & 0.5605 & 0.0056 & 0.04526 & 0.00025 &0 \\
2454603.953080 & 2.88 & 1.37 & 0.5650 & 0.0056 & 0.04553 & 0.00023 &0 \\
2454604.032740 & 0.73 & 1.37 & 0.5681 & 0.0057 & 0.04509 & 0.00023 &0 \\
2454604.127480 & 10.67 & 1.11 & 0.5574 & 0.0056 & 0.04465 & 0.00023 &0 \\
2454634.004620 & 18.92 & 1.39 & 0.5696 & 0.0057 & 0.04578 & 0.00027 &0 \\
2454634.955080 & 15.91 & 1.27 & 0.5692 & 0.0057 & 0.04497 & 0.00024 &0 \\
2454636.008750 & 5.22 & 1.27 & 0.5640 & 0.0056 & 0.04489 & 0.00024 &0 \\
2454637.993890 & 7.09 & 1.17 & 0.5844 & 0.0058 & 0.04540 & 0.00024 &0 \\
2454639.028070 & 16.66 & 1.13 & 0.5804 & 0.0058 & 0.04520 & 0.00026 &0 \\
2454640.078460 & -4.23 & 1.42 & 0.5735 & 0.0057 & 0.04514 & 0.00025 &0 \\
2454641.057270 & -5.86 & 1.26 & 0.5795 & 0.0058 & 0.04502 & 0.00027 &0 \\
2454674.987500 & -10.90 & 1.36 & 0.5579 & 0.0056 & 0.04533 & 0.00026 &0 \\
2454722.807470 & 8.80 & 1.33 & 0.6175 & 0.0062 & 0.04584 & 0.00026 &0 \\
2454723.800010 & -6.89 & 1.35 & 0.6078 & 0.0061 & 0.04595 & 0.00026 &0 \\
2454725.814550 & -5.67 & 1.25 & 0.6136 & 0.0061 & 0.04543 & 0.00026 &0 \\
2454726.848260 & 11.30 & 1.10 & 0.6089 & 0.0061 & 0.04552 & 0.00026 &0 \\
2454727.770120 & 11.64 & 1.10 & 0.6053 & 0.0061 & 0.04560 & 0.00027 &0 \\
2454727.901450 & 8.76 & 1.15 & 0.6052 & 0.0061 & 0.04566 & 0.00027 &0 \\
2454777.798730 & -0.05 & 1.42 & 0.5848 & 0.0058 & 0.04557 & 0.00022 &0 \\
2454778.784840 & 0.59 & 1.85 & 0.5740 & 0.0057 & 0.04574 & 0.00022 &0 \\
2454779.804000 & 6.05 & 1.54 & 0.5852 & 0.0059 & 0.04553 & 0.00023 &0 \\
2454790.688620 & 21.97 & 1.45 & 0.5857 & 0.0059 & 0.04554 & 0.00024 &0 \\
2454805.691490 & 13.62 & 1.39 & 0.5805 & 0.0058 & 0.04549 & 0.00021 &0 \\
2454806.706760 & -0.49 & 1.43 & 0.5696 & 0.0057 & 0.04533 & 0.00024 &0 \\
2454807.705230 & -6.52 & 1.50 & 0.5627 & 0.0056 & 0.04523 & 0.00021 &0 \\
2454808.750750 & 1.27 & 1.32 & 0.5720 & 0.0057 & 0.04504 & 0.00022 &0 \\
2454809.713030 & 10.83 & 2.21 & 0.5567 & 0.0056 & 0.04544 & 0.00023 &0 \\
2454810.705160 & 18.49 & 1.66 & 0.5671 & 0.0057 & 0.04515 & 0.00023 &0 \\
2454930.104550 & -2.17 & 2.05 & 0.5989 & 0.0060 & 0.04560 & 0.00026 &0 \\
2454955.038350 & 4.05 & 1.19 & 0.6057 & 0.0061 & 0.04556 & 0.00022 &0 \\
2454957.043290 & 4.48 & 2.59 & 0.5825 & 0.0058 & 0.04539 & 0.00021 &0 \\
2454983.996180 & -1.91 & 1.11 & 0.6458 & 0.0065 & 0.04637 & 0.00023 &0 \\
2454985.056460 & 9.36 & 1.27 & 0.6291 & 0.0063 & 0.04556 & 0.00022 &0 \\
2454987.016660 & 19.03 & 1.15 & 0.6145 & 0.0061 & 0.04607 & 0.00023 &0 \\
2454988.015580 & 6.00 & 1.30 & 0.6102 & 0.0061 & 0.04620 & 0.00022 &0 \\
2455017.084250 & 5.66 & 1.16 & 0.5923 & 0.0059 & 0.04564 & 0.00026 &0 \\
2455042.053680 & 4.20 & 1.26 & 0.6403 & 0.0064 & 0.04628 & 0.00027 &0 \\
2455042.992650 & 7.43 & 1.35 & 0.6228 & 0.0062 & 0.04650 & 0.00027 &0 \\
2455044.080400 & 9.20 & 1.47 & 0.6187 & 0.0062 & 0.04600 & 0.00029 &0 \\
2455045.055990 & 19.56 & 1.40 & 0.6097 & 0.0061 & 0.04577 & 0.00025 &0 \\
2455045.745750 & 2.31 & 2.97 & 0.5780 & 0.0058 & 0.04575 & 0.00032 &1 \\
2455045.793230 & 9.32 & 1.60 & 0.6016 & 0.0060 & 0.04607 & 0.00029 &1 \\
2455045.797510 & 8.74 & 1.74 & 0.6019 & 0.0060 & 0.04615 & 0.00029 &1 \\
2455045.801340 & 7.00 & 1.71 & 0.6022 & 0.0060 & 0.04609 & 0.00031 &1 \\
2455045.805880 & 9.31 & 1.63 & 0.6033 & 0.0060 & 0.04604 & 0.00030 &1 \\
2455045.810670 & 10.16 & 1.75 & 0.6042 & 0.0060 & 0.04616 & 0.00030 &1 \\
2455048.929860 & 5.17 & 1.43 & 0.5854 & 0.0059 & 0.04605 & 0.00029 &0 \\
2455075.760960 & 5.30 & 0.99 & 0.6465 & 0.0065 & 0.04612 & 0.00026 &0 \\
2455107.728900 & 18.61 & 2.90 & 0.6502 & 0.0065 & 0.04580 & 0.00026 &0 \\
2455192.701530 & 20.04 & 1.13 & 0.6121 & 0.0061 & 0.04550 & 0.00024 &0 \\
2455321.049540 & 2.72 & 1.06 & 0.6025 & 0.0060 & 0.04535 & 0.00023 &0 \\
2455343.910050 & 9.62 & 1.34 & 0.6015 & 0.0060 & 0.04553 & 0.00023 &1 \\
2455343.914020 & 6.42 & 1.38 & 0.6004 & 0.0060 & 0.04543 & 0.00022 &1 \\
2455343.918110 & 11.40 & 1.51 & 0.5990 & 0.0060 & 0.04547 & 0.00023 &1 \\
2455343.922020 & 9.59 & 1.30 & 0.6059 & 0.0061 & 0.04552 & 0.00022 &1 \\
2455343.925960 & 8.30 & 1.38 & 0.6046 & 0.0060 & 0.04552 & 0.00023 &1 \\
2455343.929780 & 5.79 & 1.25 & 0.6039 & 0.0060 & 0.04554 & 0.00022 &1 \\
2455343.933630 & 9.39 & 1.41 & 0.5995 & 0.0060 & 0.04559 & 0.00023 &1 \\
2455343.937510 & 12.71 & 1.37 & 0.6024 & 0.0060 & 0.04587 & 0.00024 &1 \\
2455343.941560 & 8.92 & 1.19 & 0.6034 & 0.0060 & 0.04547 & 0.00023 &1 \\
2455343.945170 & 10.37 & 1.20 & 0.6022 & 0.0060 & 0.04552 & 0.00021 &1 \\
2455343.948790 & 14.04 & 1.33 & 0.6111 & 0.0061 & 0.04573 & 0.00021 &1 \\
2455343.952430 & 11.38 & 1.30 & 0.6056 & 0.0061 & 0.04565 & 0.00023 &1 \\
2455343.956150 & 7.28 & 1.29 & 0.6031 & 0.0060 & 0.04564 & 0.00023 &1 \\
2455343.960870 & 8.27 & 1.47 & 0.6037 & 0.0060 & 0.04587 & 0.00023 &1 \\
2455343.965460 & 11.21 & 1.34 & 0.6071 & 0.0061 & 0.04580 & 0.00023 &1 \\
2455343.969560 & 9.26 & 1.32 & 0.6068 & 0.0061 & 0.04593 & 0.00023 &1 \\
2455343.973560 & 10.29 & 1.29 & 0.6067 & 0.0061 & 0.04562 & 0.00022 &1 \\
2455343.977750 & 10.25 & 1.37 & 0.6039 & 0.0060 & 0.04568 & 0.00022 &1 \\
2455343.981800 & 8.86 & 1.32 & 0.6048 & 0.0060 & 0.04555 & 0.00023 &1 \\
2455343.985770 & 10.93 & 1.38 & 0.6035 & 0.0060 & 0.04594 & 0.00022 &1 \\
2455343.989660 & 8.40 & 1.31 & 0.6046 & 0.0060 & 0.04590 & 0.00022 &1 \\
2455343.993340 & 7.71 & 1.22 & 0.6069 & 0.0061 & 0.04582 & 0.00022 &1 \\
2455343.996760 & 14.42 & 1.19 & 0.6088 & 0.0061 & 0.04597 & 0.00023 &1 \\
2455344.000020 & 11.09 & 1.34 & 0.6060 & 0.0061 & 0.04604 & 0.00023 &1 \\
2455344.003580 & 9.43 & 1.34 & 0.6046 & 0.0060 & 0.04592 & 0.00022 &1 \\
2455344.007000 & 9.10 & 1.32 & 0.6131 & 0.0061 & 0.04618 & 0.00023 &1 \\
2455344.010670 & 9.01 & 1.35 & 0.6125 & 0.0061 & 0.04612 & 0.00023 &1 \\
2455344.014480 & 11.99 & 1.29 & 0.6120 & 0.0061 & 0.04625 & 0.00022 &1 \\
2455344.018140 & 10.75 & 1.37 & 0.6173 & 0.0062 & 0.04600 & 0.00023 &1 \\
2455344.041740 & 11.62 & 1.32 & 0.6093 & 0.0061 & 0.04568 & 0.00024 &1 \\
2455344.078510 & 5.44 & 1.55 & 0.6039 & 0.0060 & 0.04566 & 0.00024 &1 \\
2455344.116100 & 5.97 & 1.46 & 0.6071 & 0.0061 & 0.04538 & 0.00023 &1 \\
2455376.068110 & 3.19 & 1.15 & 0.5983 & 0.0060 & 0.04521 & 0.00025 &0 \\
2455431.743590 & 21.31 & 1.16 & 0.6011 & 0.0060 & 0.04554 & 0.00027 &1 \\
2455431.746720 & 17.32 & 1.10 & 0.5989 & 0.0060 & 0.04567 & 0.00026 &1 \\
2455431.749750 & 19.54 & 1.16 & 0.5962 & 0.0060 & 0.04587 & 0.00028 &1 \\
2455431.821120 & 17.71 & 1.22 & 0.6110 & 0.0061 & 0.04589 & 0.00025 &1 \\
2455431.824160 & 18.43 & 1.10 & 0.6108 & 0.0061 & 0.04606 & 0.00025 &1 \\
2455431.827290 & 17.35 & 1.13 & 0.6114 & 0.0061 & 0.04581 & 0.00026 &1 \\
2455431.830380 & 15.28 & 1.21 & 0.6120 & 0.0061 & 0.04611 & 0.00026 &1 \\
2455431.833350 & 18.63 & 1.16 & 0.6102 & 0.0061 & 0.04603 & 0.00025 &1 \\
2455431.836410 & 16.08 & 1.25 & 0.6116 & 0.0061 & 0.04617 & 0.00026 &1 \\
2455431.839400 & 15.15 & 1.14 & 0.6106 & 0.0061 & 0.04599 & 0.00025 &1 \\
2455431.842380 & 17.66 & 1.14 & 0.6089 & 0.0061 & 0.04568 & 0.00026 &1 \\
2455431.845470 & 15.86 & 1.15 & 0.6121 & 0.0061 & 0.04618 & 0.00025 &1 \\
2455431.848320 & 16.37 & 1.25 & 0.6153 & 0.0062 & 0.04615 & 0.00026 &1 \\
2455431.851200 & 16.95 & 1.10 & 0.6202 & 0.0062 & 0.04627 & 0.00026 &1 \\
2455431.854090 & 17.39 & 1.11 & 0.6152 & 0.0062 & 0.04632 & 0.00025 &1 \\
2455431.857030 & 17.71 & 1.07 & 0.6132 & 0.0061 & 0.04618 & 0.00027 &1 \\
2455431.859980 & 14.01 & 1.16 & 0.6123 & 0.0061 & 0.04622 & 0.00025 &1 \\
2455431.862940 & 15.66 & 1.15 & 0.6123 & 0.0061 & 0.04615 & 0.00026 &1 \\
2455431.866130 & 17.88 & 1.10 & 0.6097 & 0.0061 & 0.04595 & 0.00026 &1 \\
2455431.869240 & 12.71 & 1.15 & 0.6082 & 0.0061 & 0.04598 & 0.00025 &1 \\
2455431.872220 & 20.07 & 1.11 & 0.6120 & 0.0061 & 0.04611 & 0.00026 &1 \\
2455431.875140 & 16.96 & 1.08 & 0.6044 & 0.0060 & 0.04615 & 0.00026 &1 \\
2455431.878170 & 16.91 & 1.26 & 0.6088 & 0.0061 & 0.04616 & 0.00026 &1 \\
2455431.881160 & 15.76 & 1.17 & 0.6053 & 0.0061 & 0.04610 & 0.00026 &1 \\
2455431.884060 & 14.64 & 1.17 & 0.6043 & 0.0060 & 0.04601 & 0.00026 &1 \\
2455431.887110 & 14.95 & 1.17 & 0.6092 & 0.0061 & 0.04601 & 0.00027 &1 \\
2455431.890100 & 10.42 & 1.31 & 0.6110 & 0.0061 & 0.04598 & 0.00025 &1 \\
2455431.893070 & 14.67 & 1.15 & 0.6105 & 0.0061 & 0.04620 & 0.00026 &1 \\
2455431.896060 & 15.81 & 1.18 & 0.6075 & 0.0061 & 0.04610 & 0.00025 &1 \\
2455431.899050 & 16.48 & 1.16 & 0.6072 & 0.0061 & 0.04608 & 0.00026 &1 \\
2455431.902040 & 14.67 & 1.16 & 0.6030 & 0.0060 & 0.04609 & 0.00026 &1 \\
2455431.905020 & 15.09 & 1.18 & 0.6051 & 0.0061 & 0.04604 & 0.00026 &1 \\
2455431.907970 & 16.31 & 1.19 & 0.6011 & 0.0060 & 0.04614 & 0.00026 &1 \\
2455431.910960 & 15.28 & 1.08 & 0.6044 & 0.0060 & 0.04603 & 0.00026 &1 \\
2455431.913970 & 10.54 & 1.13 & 0.6053 & 0.0061 & 0.04607 & 0.00025 &1 \\
2455431.916980 & 12.65 & 1.24 & 0.6046 & 0.0060 & 0.04612 & 0.00026 &1 \\
2455431.920000 & 11.23 & 1.15 & 0.6024 & 0.0060 & 0.04617 & 0.00026 &1 \\
2455431.923100 & 14.43 & 1.25 & 0.6008 & 0.0060 & 0.04629 & 0.00026 &1 \\
2455431.926350 & 15.17 & 1.25 & 0.5994 & 0.0060 & 0.04614 & 0.00026 &1 \\
2455431.929540 & 12.73 & 1.26 & 0.5989 & 0.0060 & 0.04587 & 0.00025 &1 \\
2455431.932680 & 14.29 & 1.25 & 0.6017 & 0.0060 & 0.04597 & 0.00026 &1 \\
2455431.935930 & 10.77 & 1.11 & 0.6019 & 0.0060 & 0.04608 & 0.00027 &1 \\
2455431.939180 & 13.57 & 1.14 & 0.6013 & 0.0060 & 0.04597 & 0.00026 &1 \\
2455431.942370 & 14.52 & 1.20 & 0.6010 & 0.0060 & 0.04603 & 0.00025 &1 \\
2455431.945520 & 12.45 & 1.20 & 0.6020 & 0.0060 & 0.04613 & 0.00026 &1 \\
2455431.948750 & 9.86 & 1.17 & 0.6013 & 0.0060 & 0.04582 & 0.00025 &1 \\
2455431.952030 & 13.72 & 1.19 & 0.6086 & 0.0061 & 0.04608 & 0.00025 &1 \\
2455431.955310 & 12.52 & 1.34 & 0.6050 & 0.0060 & 0.04605 & 0.00025 &1 \\
2455431.958700 & 12.72 & 1.18 & 0.6041 & 0.0060 & 0.04572 & 0.00025 &1 \\
2455431.962210 & 14.32 & 1.10 & 0.6035 & 0.0060 & 0.04567 & 0.00026 &1 \\
2455431.965690 & 11.75 & 1.27 & 0.5995 & 0.0060 & 0.04588 & 0.00025 &1 \\
2455431.969140 & 11.29 & 1.22 & 0.5954 & 0.0060 & 0.04569 & 0.00026 &1 \\
2455431.972470 & 13.05 & 1.20 & 0.5988 & 0.0060 & 0.04592 & 0.00025 &1 \\
2455431.975860 & 14.14 & 1.27 & 0.5991 & 0.0060 & 0.04605 & 0.00024 &1 \\
2455431.979180 & 12.32 & 1.23 & 0.5992 & 0.0060 & 0.04605 & 0.00026 &1 \\
2455431.982500 & 12.00 & 1.15 & 0.6001 & 0.0060 & 0.04594 & 0.00026 &1 \\
2455431.985830 & 15.03 & 1.22 & 0.5993 & 0.0060 & 0.04578 & 0.00026 &1 \\
2455431.989190 & 11.21 & 1.17 & 0.5973 & 0.0060 & 0.04605 & 0.00026 &1 \\
2455431.992520 & 7.84 & 1.25 & 0.5966 & 0.0060 & 0.04595 & 0.00026 &1 \\
2455431.995790 & 10.88 & 1.18 & 0.5981 & 0.0060 & 0.04595 & 0.00025 &1 \\
2455431.999200 & 11.61 & 1.15 & 0.5971 & 0.0060 & 0.04566 & 0.00026 &1 \\
2455432.002440 & 13.38 & 1.24 & 0.5995 & 0.0060 & 0.04593 & 0.00026 &1 \\
2455432.005680 & 11.29 & 1.18 & 0.5950 & 0.0059 & 0.04571 & 0.00026 &1 \\
2455432.008970 & 14.39 & 1.16 & 0.6016 & 0.0060 & 0.04566 & 0.00026 &1 \\
2455432.012160 & 10.37 & 1.18 & 0.6062 & 0.0061 & 0.04590 & 0.00026 &1 \\
2455432.015450 & 10.04 & 1.18 & 0.6000 & 0.0060 & 0.04571 & 0.00025 &1 \\
2455432.018610 & 15.34 & 1.16 & 0.5980 & 0.0060 & 0.04571 & 0.00025 &1 \\
2455432.021810 & 15.49 & 1.16 & 0.6010 & 0.0060 & 0.04577 & 0.00027 &1 \\
2455432.057450 & 7.23 & 1.35 & 0.6004 & 0.0060 & 0.04544 & 0.00027 &1 \\
2455432.059850 & 10.65 & 1.40 & 0.5923 & 0.0059 & 0.04525 & 0.00026 &1 \\
2455432.062340 & 8.16 & 1.41 & 0.5768 & 0.0058 & 0.04535 & 0.00026 &1 \\
2455469.781030 & 22.81 & 1.17 & 0.6103 & 0.0061 & 0.04632 & 0.00027 &0 \\
2455706.943110 & 2.79 & 1.17 & 0.5949 & 0.0059 & 0.04591 & 0.00023 &0 \\
2455843.873950 & 7.91 & 1.41 & 0.6089 & 0.0061 & 0.04569 & 0.00023 &0 \\
2455903.710580 & 20.90 & 1.41 & 0.5773 & 0.0058 & 0.04595 & 0.00023 &0 \\
2456165.062090 & 18.33 & 1.39 & 0.5879 & 0.0059 & 0.04459 & 0.00024 &0 \\
2456167.038410 & 5.65 & 1.23 & 0.5827 & 0.0058 & 0.04527 & 0.00026 &0 \\
2456450.111570 & 0.31 & 1.20 & 0.5575 & 0.0056 & 0.04537 & 0.00022 &0 \\
2456487.122080 & 21.92 & 1.48 & 0.5786 & 0.0058 & 0.04628 & 0.00024 &0 \\
2456494.933410 & 9.60 & 1.32 & 0.6316 & 0.0063 & 0.04668 & 0.00027 &0 \\
2456846.854840 & -40.68 & 1.43 & 0.6050 & 0.0060 & 0.04544 & 0.00026 &0 \\
2456860.910650 & -53.08 & 1.63 & 0.5801 & 0.0058 & 0.04613 & 0.00030 &0 \\
2456861.977640 & -45.69 & 1.47 & 0.5930 & 0.0059 & 0.04542 & 0.00032 &0 \\
2456862.967090 & -28.42 & 1.48 & 0.5805 & 0.0058 & 0.04489 & 0.00029 &0 \\
2456864.080510 & -43.08 & 1.61 & 0.6025 & 0.0060 & 0.04554 & 0.00030 &0 \\
2456865.122640 & -38.00 & 1.48 & 0.5979 & 0.0060 & 0.04565 & 0.00029 &0 \\
2456866.112220 & -40.79 & 1.69 & 0.6044 & 0.0060 & 0.04557 & 0.00028 &0 \\
2456867.079570 & -31.60 & 1.69 & 0.6150 & 0.0062 & 0.04531 & 0.00026 &0 \\
2456872.958960 & -25.40 & 1.45 & 0.6252 & 0.0063 & 0.04552 & 0.00027 &0 \\
2456880.778860 & -42.19 & 1.35 & 0.5996 & 0.0060 & 0.04557 & 0.00028 &0 \\
2456881.755090 & -39.70 & 1.56 & 0.5967 & 0.0060 & 0.04588 & 0.00028 &0 \\
2456883.010490 & -33.55 & 1.38 & 0.5900 & 0.0059 & 0.04582 & 0.00026 &0 \\
2456884.013280 & -47.75 & 1.37 & 0.5894 & 0.0059 & 0.04560 & 0.00025 &0 \\
2456889.047530 & -57.41 & 1.31 & 0.5371 & 0.0054 & 0.04505 & 0.00026 &0 \\
2456891.915060 & -49.74 & 1.36 & 0.5266 & 0.0053 & 0.04529 & 0.00025 &0 \\
2456893.047790 & -36.49 & 1.41 & 0.5326 & 0.0053 & 0.04527 & 0.00027 &0 \\
2456895.056280 & -53.60 & 1.40 & 0.5755 & 0.0058 & 0.04543 & 0.00028 &0 \\
2456907.021220 & -34.98 & 1.54 & 0.5898 & 0.0059 & 0.04512 & 0.00026 &0 \\
2456908.011260 & -46.67 & 1.44 & 0.5678 & 0.0057 & 0.04504 & 0.00026 &0 \\
2456908.873170 & -50.18 & 1.42 & 0.5635 & 0.0056 & 0.04503 & 0.00027 &0 \\
2456909.998860 & -56.69 & 1.45 & 0.5582 & 0.0056 & 0.04524 & 0.00026 &0 \\
2456910.953780 & -44.77 & 1.46 & 0.5669 & 0.0057 & 0.04543 & 0.00027 &0 \\
2456912.019380 & -34.52 & 1.56 & 0.5622 & 0.0056 & 0.04544 & 0.00026 &0 \\
2457000.741630 & -40.21 & 1.47 & 0.5611 & 0.0056 & 0.04504 & 0.00022 &0 \\
2457001.734690 & -55.37 & 1.39 & 0.5581 & 0.0056 & 0.04566 & 0.00024 &0 \\
2457002.708900 & -54.45 & 1.50 & 0.5547 & 0.0055 & 0.04540 & 0.00024 &0 \\
2457151.129480 & -19.58 & 1.35 & 0.5240 & 0.0052 & 0.04578 & 0.00024 &0 \\
2457180.124130 & -21.46 & 1.44 & 0.5632 & 0.0056 & 0.04567 & 0.00023 &0 \\
2457202.884560 & -40.46 & 1.44 & 0.5120 & 0.0051 & 0.04571 & 0.00025 &0 \\
2457208.116140 & -34.50 & 1.50 & 0.5331 & 0.0053 & 0.04584 & 0.00027 &0 \\
2457216.004270 & -24.86 & 1.42 & 0.5506 & 0.0055 & 0.04485 & 0.00030 &0 \\
2457218.118600 & -39.34 & 1.39 & 0.5345 & 0.0053 & 0.04516 & 0.00025 &0 \\
2457233.104170 & -32.99 & 1.53 & 0.5018 & 0.0050 & 0.04500 & 0.00035 &0 \\
2457234.109800 & -21.35 & 1.37 & 0.5094 & 0.0051 & 0.04499 & 0.00029 &0 \\
2457237.079710 & -33.48 & 1.42 & 0.5306 & 0.0053 & 0.04524 & 0.00027 &0 \\
2457241.100990 & -26.61 & 1.41 & 0.5366 & 0.0054 & 0.04514 & 0.00026 &0 \\
2457247.084080 & -40.98 & 1.48 & 0.5329 & 0.0053 & 0.04496 & 0.00029 &0 \\
2457296.962090 & -29.38 & 1.44 & 0.4851 & 0.0049 & 0.04489 & 0.00023 &0 \\
2457326.846390 & -20.30 & 1.66 & 0.4740 & 0.0047 & 0.04577 & 0.00020 &0 \\
2457353.790300 & -32.25 & 1.53 & 0.4743 & 0.0047 & 0.04519 & 0.00020 &0 \\
2457355.776030 & -22.95 & 1.46 & 0.4714 & 0.0047 & 0.04527 & 0.00023 &0 \\
2457378.705940 & -38.71 & 1.51 & 0.5485 & 0.0055 & 0.04624 & 0.00024 &0 \\
2457598.973200 & -22.62 & 1.56 & 0.4540 & 0.0045 & 0.04547 & 0.00025 &0 \\
2457703.790140 & -2.26 & 1.54 & 0.5034 & 0.0050 & 0.04600 & 0.00021 &0 \\
2457829.111270 & -11.39 & 1.48 & 0.5391 & 0.0054 & 0.04528 & 0.00026 &0 \\
2457830.148270 & -2.44 & 1.44 & 0.5229 & 0.0052 & 0.04494 & 0.00025 &0 \\
2457831.120920 & 11.13 & 1.43 & 0.5245 & 0.0052 & 0.04517 & 0.00028 &0 \\
2457853.138650 & -16.51 & 1.51 & 0.5702 & 0.0057 & 0.04559 & 0.00023 &0 \\
2457855.120060 & 6.02 & 1.47 & 0.5529 & 0.0055 & 0.04514 & 0.00024 &0 \\
2457888.078440 & -9.35 & 1.22 & 0.5124 & 0.0051 & 0.04501 & 0.00022 &0 \\
2457911.987050 & -16.72 & 1.26 & 0.5400 & 0.0054 & 0.04605 & 0.00025 &0 \\
2457923.987270 & 11.24 & 1.38 & 0.5576 & 0.0056 & 0.04486 & 0.00026 &0 \\
2457923.987270 & 11.24 & 1.38 & 0.5576 & 0.0056 & 0.04486 & 0.00026 &0 \\
2457925.078110 & -5.13 & 1.55 & 0.5639 & 0.0056 & 0.04530 & 0.00023 &0 \\
2457927.053500 & 2.49 & 1.31 & 0.5806 & 0.0058 & 0.04641 & 0.00025 &0 \\
2457933.012170 & 18.08 & 1.31 & 0.6256 & 0.0063 & 0.04608 & 0.00025 &0 \\
2457940.004810 & -13.19 & 1.37 & 0.5548 & 0.0055 & 0.04643 & 0.00027 &0 \\
2457943.958790 & 0.13 & 1.45 & 0.5398 & 0.0054 & 0.04630 & 0.00027 &0 \\
2457946.046760 & -9.17 & 1.45 & 0.5446 & 0.0054 & 0.04533 & 0.00026 &0 \\
2457963.852410 & 14.62 & 1.44 & 0.5876 & 0.0059 & 0.04605 & 0.00034 &0 \\
2457971.883100 & -5.76 & 1.25 & 0.5188 & 0.0052 & 0.04664 & 0.00025 &0 \\

